Implicit Surface Reconstruction with a Curl-free Radial Basis Function Partition of Unity Method

Surface reconstruction from a set of scattered points, or a point cloud, has many applications ranging from computer graphics to remote sensing. We present a new method for this task that produces an implicit surface (zero-level set) approximation for an oriented point cloud using only information about (approximate) normals to the surface. The technique exploits the fundamental result from vector calculus that the normals to an implicit surface are curl-free. By using a curl-free radial basis function (RBF) interpolation of the normals, we can extract a potential for the vector field whose zero-level surface approximates the point cloud. We use curl-free RBFs based on polyharmonic splines for this task, since they are free of any shape or support parameters. Furthermore, to make this technique efficient and able to better represent local sharp features, we combine it with a partition of unity (PU) method. The result is the curl-free partition of unity (CFPU) method. We show how CFPU can be adapted to enforce exact interpolation of a point cloud and can be regularized to handle noise in both the normal vectors and the point positions. Numerical results are presented that demonstrate how the method converges for a known surface as the sampling density increases, how regularization handles noisy data, and how the method performs on various problems found in the literature.

==> arxiv 2/macros.tex <==
\newcommand{\tand}{\textnormal{and}}
\newcommand{\ot}{\otimes}
\newcommand{\hn}{\hat{\mathbf{n}}}
\newcommand{\ep}{\varepsilon}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\lat}{\theta}
\newcommand{\lon}{\lambda}
\newcommand{\latv}{\gamma}
\newcommand{\lonu}{\delta}

\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vst}{\widetilde{\mathbf{s}}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\pts}{\mathbf{x}}
\newcommand{\Pts}{X}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vxn}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
%\newcommand{\vom}{\boldsymbol{\omega}}
\newcommand{\vom}{\boldsymbol{\xi}}
\newcommand{\vtheta}{\boldsymbol{\theta}}
\newcommand{\vxi}{\boldsymbol{\xi}}
\newcommand{\nrml}{\mathbf{n}}
\newcommand{\prad}{\rho}

\newcommand{\vzero}{\mathbf{0}}

\newcommand{\vlambda}{\mathbf{\lambda}}


\newcommand{\vF}{\mathbf{F}}
\newcommand{\vH}{\mathbf{H}}
\newcommand{\vtH}{\widetilde{\mathbf{H}}}
\newcommand{\tH}{\widetilde{H}}
\newcommand{\tpsi}{\widetilde{\psi}}
\newcommand{\vI}{\mathbf{I}}
\newcommand{\vL}{\mathbf{L}}
\newcommand{\vQ}{\mathbf{Q}}
\newcommand{\vP}{\mathbf{P}}
\newcommand{\rot}{\mathbf{L}}
%\newcommand{\sgrad}{\nabla^{*}}
\newcommand{\sgrad}{\mathbf{G}}

\newcommand{\rhat}{\widehat{\vr}}
\newcommand{\thetahat}{\widehat{\vtheta}}
\newcommand{\zhat}{\widehat{\vz}}


\newcommand{\calE}{\mathcal{E}}
\newcommand{\M}{\mathcal{P}}

\newcommand{\vcurl}{\textnormal{\textbf{curl}}}
\newcommand{\scurl}{\textnormal{curl}}
\newcommand{\spheregrad}{{\nabla_{\sphere^2}}}
\newcommand{\spherecurl}{\mathcal{L}}
\newcommand{\sspherecurl}{\textnormal{curl}_{\sphere^2}}
\newcommand{\vspherecurl}{\textnormal{\textbf{curl}}_{\sphere^2}}
\newcommand{\Phidiv}{\Phi_{\rm div}}
\newcommand{\Phidivt}{\widetilde{\Phi}_{\rm div}}
%\newcommand{\Phicurl}{\Phi_{\rm curl}}
%\newcommand{\Phicurlt}{\widetilde{\Phi}_{\rm curl}}
\newcommand{\Phicurl}{\Phi}
\newcommand{\Phicurlt}{\widetilde{\Phi}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\dist}{\textnormal{dist}}
\newcommand{\sdist}{\textnormal{dist}_{\surface}}


\definecolor{matred}{rgb}{0.6350, 0.0780, 0.1840}
\definecolor{matblue}{rgb}{0, 0.4470, 0.7410}
\definecolor{matpurp}{rgb}{0.4940, 0.1840, 0.5560}
\definecolor{matgreen}{rgb}{0, 0.5, 0}

\newcommand{\dfcylkernel}{K_{div}}
\newcommand{\cfcylkernel}{K_{curl}}
\newcommand{\dfpuapprox}{\widetilde{\vs}}
\newcommand{\cfpot}{s}  % cf potential for the vector approximant
\newcommand{\tcfpot}{f}  % target cf potential
\newcommand{\mcfpot}{\overline{\cfpot}}  % cf potential for the vector approximant with mean zero
\newcommand{\icfpot}{\widetilde{\cfpot}}  % cf potential for the vector approximant that exactly interpolates
\newcommand{\dfpot}{\psi}
\newcommand{\dfvpot}{\boldsymbol{\psi}}
\newcommand{\blendedcfpot}{\cfpot}
\newcommand{\blendeddfpot}{\widetilde{\dfpot}}
\newcommand{\localadjdfpot}{\widetilde{\dfpot}}
\newcommand{\localadjcfpot}{\widetilde{\cfpot}}
\newcommand{\blendedpotential}{\widetilde{\dfpot}}
\newcommand{\localadjpotential}{\widetilde{\dfpot}}

\newcommand{\gluept}{\bar{\vx}}
\newcommand{\patch}{\Omega}
\newcommand{\glueptset}{\bar{X}}
\newcommand{\shift}{b}
\newcommand{\rhs}{c}
\newcommand{\res}{r}
\newcommand{\nodeset}{X}
\newcommand{\node}{\mathbf{x}}
\newcommand{\surface}{\mathcal{P}}
\newcommand{\surfacegrad}{\mathbf{G}}
\newcommand{\surfacecurl}{\mathbf{L}}


\definecolor{mygreen}{rgb}{0.13,0.54,0.13}
\definecolor{purple}{rgb}{0.5412,0.1686,0.8863}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\ds}{\displaystyle}
%\newcommand{\gcomment}[1]{{\color{red}[GBW: #1]}}
%\newcommand{\ecomment}[1]{{\color{blue}[EJF: #1]}}
%\newcommand{\ecomment}[1]{{}}
\newcommand{\revision}[1]{{\color{black}#1}}
\newcommand{\refone}[1]{{\color{black}#1}}
\newcommand{\reftwo}[1]{{\color{black}#1}}

\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

